Scalable Graph Compressed Convolutions

Designing effective graph neural networks (GNNs) with message passing has two fundamental challenges, i.e., determining optimal message-passing pathways and designing local aggregators. Previous methods of designing optimal pathways are limited with information loss on the input features. On the other hand, existing local aggregators generally fail to extract multi-scale features and approximate diverse operators under limited parameter scales. In contrast to these methods, Euclidean convolution has been proven as an expressive aggregator, making it a perfect candidate for GNN construction. However, the challenges of generalizing Euclidean convolution to graphs arise from the irregular structure of graphs. To bridge the gap between Euclidean space and graph topology, we propose a differentiable method that applies permutations to calibrate input graphs for Euclidean convolution. The permutations constrain all nodes in a row regardless of their input order and therefore enable the flexible generalization of Euclidean convolution to graphs. Based on the graph calibration, we propose the Compressed Convolution Network (CoCN) for hierarchical graph representation learning. CoCN follows local feature-learning and global parameter-sharing mechanisms of convolution neural networks. The whole model can be trained end-to-end, with compressed convolution applied to learn individual node features and their corresponding structure features. CoCN can further borrow successful practices from Euclidean convolution, including residual connection and inception mechanism. We validate CoCN on both node-level and graph-level benchmarks. CoCN achieves superior performance over competitive GNN baselines. Codes are available at https://github.com/sunjss/CoCN.

==> fig-tex/app-kernel-layer.tex <==
\begin{figure*}[htb]
\centering
\includegraphics[width=0.5\textwidth]{fig/kernel-layer-MUTAG.pdf}
\vskip -0.1in
\caption{\textbf{Ablation Study on the Kernel Size and Receptive Field Size for MUTAG.} The dashed line represents the average number of nodes for all graphs. The dotted line represents the maximum number of nodes in one graph.}
\label{fig:app-kernel-layer}
\end{figure*}

==> latexmkrc <==
# This shows how to use the xr package with latexmk.
# John Collins 2023-03-29
#
# The xr package ("a system for eXternal References") is used by a document
# to make references to sections, equations, etc in other external
# documents. 
# The definitions in this file enable latexmk to apply latexmk to
# automatically update an external document whenever its .tex file changes,
# so that the references in the main document stay up to date.

# Notes:
#    1. This version is defined to put the files from the compilations of
#       the external documents into a defined subdirectory, to segregate
#       potentially many generated files from the main document
#       directories. 
#    2. But for latexmk's custom dependency mechanism to be used, as here,
#       the aux file from compilation of a subdocument must be generated in
#       the same directory as the corresponding source .tex file.  So the
#       .aux file is copied.
#    3. It is assumed that the external documents are to be compiled by
#       pdflatex.  This can be changed, of course, by changing the '-pdf'
#       option given to the invoked latexmk to whatever is needed.
#    4. An ideal implementation would also ensure that recompilation of an
#       external document also happens whenever any of its other source
#       files changes.  But this is not done in the present version, and
#       would probably entail either the use of internal latexmk variables
#       or extra enhancements to latexmk.
#    5. The code uses subroutines copy and fileparse that are loaded by
#       latexmk from the Perl packages File::Copy and File::Basename.
#    6. It also uses some not-yet-documented features of latexmk: an array
#       variable @file_not_found and subroutines popd, pushd, and
#       rdb_add_generated. 


#--------------------
# Configurable choices for compilation of external documents

# Subdirectory for output files from compilation of external documents:
$sub_doc_output = 'output-subdoc';

# Options to supply to latexmk for compilation of external documents:
@sub_doc_options = ();

push @sub_doc_options, '-pdf'; # Use pdflatex for compilation of external documents.
# Replace '-pdf' by '-pdfdvi', 'pdfxe', or 'pdflua' if needed.

#--------------------

# Add a pattern for xr's log-file message about missing files to latexmk's
# list.  Latexmk's variable @file_not_found is not yet documented.
# This line isn't necessary for v. 4.80 or later of latexmk.
push @file_not_found, '^No file\\s*(.+)\s*$';

add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );
sub makeexternaldocument {
    if ( $root_filename ne $_[0] )  {
        my ($base_name, $path) = fileparse( $_[0] );
        pushd $path;
        my $return = system "latexmk",
                            @sub_doc_options,
                            "-aux-directory=$sub_doc_output",
                            "-output-directory=$sub_doc_output",
                            $base_name;
        if ( ($sub_doc_output ne ' ') && ($sub_doc_output ne '.') ) {
               # In this case, .aux file generated by pdflatex isn't in same
               # directory as the .tex file.
               # Therefore:
               # 1. Actual generated aux file must be listed as produced by this
               #    rule, so that latexmk deals with dependencies correctly.
               #    (Problem to overcome: If $sub_dir_output is same as $aux_dir
               #    for the main document, xr may read the .aux file in the
               #    aux_dir rather than the one the cus dep is assumed by latexmk
               #    to produce, which is in the same directory as the .tex source
               #    file for this custom dependency.)
               #    Use not-yet-documented latexmk subroutine rdb_add_generated
               #    to do this:
               # 2. A copy of the .aux file must be in same directory as .tex file
               #    to satisfy latexmk's definition of a custom dependency.
             rdb_add_generated( "$sub_doc_output/$base_name.aux" );
             copy "$sub_doc_output/$base_name.aux", ".";
        }
        popd;
        return $return;
   }
}

==> tab-tex/app-ablation-feat.tex <==
\begin{table*}[hbp]
% \vskip -2in
\caption{\textbf{Ablation Study on Structure Features and Node Features for Graph Classification Datasets (measured by accuracy: \%).}}
\vskip 0.1in
\label{tab:ablation-feat-graph}
\begin{center}
\begin{small}
\begin{sc}
\begin{tabular}{lcccccccccccc} 
\toprule
          & MUTAG & PROTEINS & NCI1  & IMDB-B & IMDB-M & COLLAB  \\ 
\hline
Str. Feat.  & \textbf{88.35} & 72.03    & 64.08 & 70.47  & 48.16  & 78.14\\
Nod. Feat. & 85.12 & 76.22    & 78.65 & 76.17  & 54.03  & 84.46  \\ 
% \hline
Both      & 87.08 & \textbf{76.86}    & \textbf{82.28} & \textbf{77.26}  & \textbf{56.32}  & \textbf{86.15}\\
\bottomrule
\end{tabular}
\end{sc}
\end{small}
\end{center}

\vskip 0.2in
\caption{\textbf{Ablation Study on Structure Features and Node Features for Node Classification Datasets (measured by accuracy: \%).}}
\vskip 0.1in
\label{tab:ablation-feat-node}
\begin{center}
\begin{small}
\begin{sc}
\begin{tabular}{lcccccccccccc} 
\toprule
          & Chameleon & Squirrel & Cornell & Texas & Wisconsin & Actor  \\ 
\hline
Str. Feat.  & 67.82     & 72.79    & 66.22   & 72.16 & 79.23     & 33.73  \\
Nod. Feat. & 77.98     & 71.91    & 79.19   & 79.41 & 83.53     & 34.36  \\ 
% \hline
Both      & \textbf{79.17}     & \textbf{72.95}    & \textbf{81.08}   & \textbf{80.54} & \textbf{84.90}     & \textbf{35.55}  \\
\bottomrule
\end{tabular}
\end{sc}
\end{small}
\end{center}
\end{table*}

==> tab-tex/app-ablation-l1.tex <==
\begin{table*}[t]
\begin{center}
\caption{\textbf{Ablation Study on $L_1$ (measured by accuracy: \%).}}\label{tab:ablation-l1}
\vskip 0.1in
\begin{small}
\begin{sc}
\begin{tabular}{lccccccc} 
\toprule
          & 1              & 2     & 3     & 4     & 6     & 8     & 10     \\ 
\hline
Chameleon & \textbf{79.25} & 78.86 & 78.81 & 79.08 & 78.64 & 77.94 & 77.74  \\
MUTAG     & \textbf{87.08} & 86.06 & 86.60 & 85.27 & 84.58 & 84.79 & 84.62  \\
\bottomrule
\end{tabular}
\end{sc}
\end{small}
\end{center}
\end{table*}

==> tab-tex/app-ablation-t.tex <==
\begin{table*}[t]
\begin{center}
\caption{\textbf{Ablation Study on Smoothness Parameter $t$ (measured by accuracy: \%).}}\label{tab:ablation-t}
\vskip 0.1in
\begin{small}
\begin{sc}
\begin{tabular}{lcccccc} 
\toprule
          & 0              & 1              & 2     & 4     & 6     & 8               \\ 
\hline
Chameleon & 49.45          & \textbf{78.39} & 77.26 & 76.63 & 75.77 & 74,04           \\
Cornell   & \textbf{82.16} & 75.95          & 76.49 & 75.95 & 75.14 & 72.43           \\
MUTAG     & 85.09          & 85.94          & 85.84 & 86.62 & 86.51 & \textbf{87.19}  \\
\bottomrule
\end{tabular}
\end{sc}
\end{small}
\end{center}
\end{table*}

==> tab-tex/app-node-degree.tex <==
\begin{table*}[t]
\caption{\textbf{Statistics on Average Degree.}}
\label{tab:degree}
\vskip 0.1in
\begin{center}
\begin{small}
\begin{sc}
\begin{tabular}{lcccccc} 
\toprule
           & MUTAG     & PROTEINS & NCI1    & IMDB-B & IMDB-M    & COLLAB  \\
Avg Degree & 4         & 7        & 4       & 39     & 40        & 263     \\ 
\hline
           & Chameleon & Squirrel & Cornell & Texas  & Wisconsin & Actor   \\
Avg Degree & 15.85     & 41.74    & 1.63    & 1.78   & 2.05      & 3.95    \\
\bottomrule
\end{tabular}
\end{sc}
\end{small}
\end{center}
\end{table*}
